Implicit Coordination using Active Epistemic Inference for Multi-Robot Systems

A Multi-robot system (MRS) provides significant advantages for intricate tasks such as environmental monitoring, underwater inspections, and space missions. However, addressing potential communication failures or the lack of communication infrastructure in these fields remains a challenge. A significant portion of MRS research presumes that the system can maintain communication with proximity constraints, but this approach does not solve situations where communication is either non-existent, unreliable, or poses a security risk. Some approaches tackle this issue using predictions about other robots while not communicating, but these methods generally only permit agents to utilize first-order reasoning, which involves reasoning based purely on their own observations. In contrast, to deal with this problem, our proposed framework utilizes Theory of Mind (ToM), employing higher-order reasoning by shifting a robot's perspective to reason about a belief of others observations. Our approach has two main phases: i) an efficient runtime plan adaptation using active inference to signal intentions and reason about a robot's own belief and the beliefs of others in the system, and ii) a hierarchical epistemic planning framework to iteratively reason about the current MRS mission state. The proposed framework outperforms greedy and first-order reasoning approaches and is validated using simulations and experiments with heterogeneous robotic systems.

==> old_formulation_scratch.tex <==
The last tensor, $A_i^J$ the joint likelihood of a hidden state, assuming that the evidences are independent:
Given the general definitions for the set $M$ of tensors that describe the generative model, we can now explicitly discuss the mapping between the hidden state $\tilde{s}$ for each robot by first defining the first-order reasoning about the state of the system. $\bm{D}_i$ is initialized by the prior information that a robot $i$ knows about the system. For example, if the robots initially know the starting locations of all robots in the system, we can write this as $\bm{D}_i = \bigotimes_{k=1}^m D_i^k$.

The matrix $\bm{C}$ encodes a preference for a specific configuration or set of configurations. $\bm{C}$ does not include a subscript and must be known to the entire system in advance. $\bm{C} = C_1\otimes C_2 \otimes C_3$ is defined by observation preferences such as moving toward a goal ($C_1$), mission preferences such as preferring certain robots to achieve certain goals ($C_2$), and mission objectives such as minimizing energy consumption ($C_3)$ where we assume that the tensors associated with $\bm{C}$ are one-hot encodings for discrete evaluation of the operational preferences. The matrix $\bm{B}_i$ encodes the probability of transitioning from one state to another given a control input $\bm{u}_i$ for a robot $i$. In this MRS application, $\bm{B}_i$ maps how predicted observations will change the belief over the hidden states for a control input. Lastly, $\bm{A}_i$ encodes the likelihood that a robot $i$'s observations correlate with a belief about a hidden state. For a heterogeneous robotic system, $\bm{A}_i$ correlates with a robot $i$'s measurement model in the state estimation process and how evidence can be gathered from a measurement and mapped to a likelihood. The likelihood mapping between the hidden states $\tilde{S}_i$ and observations $\bm{o}_i$ is specified using a 3-order tensor where $\bm{A}_i = A^0_i\otimes A^1_i \otimes A^J_i$.

The first tensor $A_i^0$ maps a hidden state that represents the position of a robot to its self-observations. Then these observations are assessed using a salience function~\cite{parr2017working} that evaluates the evidence that a robot is pursuing a goal given the observations. The salience function is given by a generalized exponential function:
\begin{equation}
    \upsilon^i_{\tilde{s}} = \beta \exp\left(-\frac{1}{\eta} \bm{h}_s(\bm{o}_i)\right)
\end{equation}
where $\beta,\eta$ are constants that defines the proportionality of the evidence associated with the observation $\bm{o}_i$ and the hidden state $\tilde{s}$. The function $\bm{h}_0(\cdot)\in\R^+$ is a general function that evaluates a positive value associated with a robot's self-observation. To obtain the likelihood, we let:
\begin{equation}
    P(\bm{o}^i_{i} \ | \ \tilde{s}) = \sigma(\upsilon^i_{\tilde{s}})
\end{equation}
where $\sigma(\cdot)$ is the numerically stable softmax function such that:
\begin{equation}
    \sigma(\upsilon^i)_{\tilde{s}} = \frac{\exp(\upsilon^i_{\tilde{s}}-\max(\upsilon^i_{\tilde{S}}))}{\sum_{\tilde{q}\in\tilde{S}} \exp(\upsilon^i_{\tilde{q}} - \max(\upsilon^i_{\tilde{S}}))}
\end{equation}

The second tensor, $A_i^1$, maps a hidden state that represents the position of other robots to their observations. Using a similar salience function, but considering the measurement model for robot $i$ denoted as $\omega_i$, we let the evidence associated with a robot $j$ perceived by robot $i$ to be pursuing any goal to be formulated as:
\begin{equation}
    \upsilon^j_{\tilde{s}} = \beta \exp\left(-\frac{1}{\eta} \bm{h}_1(\bm{o}_i,\omega_i)\right)
\end{equation}
where the function $\bm{h}_1(\cdot)\in\R^+$ is a general function that evaluates a positive value associated with a robot's observation of another robot in the MRS.



\begin{equation}
    A^J_{i\hspace{1pt} {\tilde{s}}} = P(\bm{o}_i \ | \ \tilde{s}) \equiv \prod_{j = 1}^m \upsilon^j_{\tilde{s}}
\end{equation}
The result is a mapping from an observation $\bm{o}_i$ for robot $i$ about themselves and their observations about other robots in the system before computing a joint probability model for each goal configuration in the set $\tilde{S}$. Using these computations, we can evaluate expected free energy over the goal configurations for a robot policy $\pi$ such that:
\begin{equation}
    \bm{G}_t(\pi_{it}) = \sum_{\tau = t}^T\mathbb{E}_{Q(\tilde{S} | \pi_{i})}\left[-\ln \bm{A}_{it} - \ln \bm{C}_{it}\right]
\end{equation}

We observe that while this provides a comprehensive approach for employing active inference in a multi-robot system with continuous observations and controls and no explicit communication, the diverse nature of an MRS inherently introduces a variety of capabilities and measurement models for different vehicle types. To take advantage of this, we incorporate higher-order reasoning into the active inference framework.

\subsubsection{Higher-order Reasoning}\label{sec:higherorder}
As discussed in Sec.~\ref{sec:firstorder}, first-order reasoning enables the robot to determine its posterior belief from its own viewpoint. In contrast, higher-order reasoning allows a robot to understand and consider the estimated perceptions of other robots within the system. Within the framework of the active inference model, the inclusion of higher-order reasoning enhances the estimation of expected free energy by integrating the measurable perceptions of other robots into the policy-perception loop.

To accomplish higher-order reasoning in the active inference framework, we introduce two new tensors, $A_i^2$ and $A_i^3$, to the tensorial product $\bm{A}_i$ such that $\bm{A}_i = \left(\bigotimes_{k = 0}^3 A^k_i \right)\otimes A_i^J$. Initially, the tensor $A_i^2$ maps the result from $A_i^0$ to an observation of how other robots perceive the position of robot $i$ from its own viewpoint. This allows the system to integrate second-order reasoning within the active inference framework. Subsequently, the tensor $A_i^3$ maps the result from $A_i^1$ to an observation about how other robots perceive each other from the viewpoint of the robot $i$, thus incorporating third-order reasoning. 
